How To Train Your Deep Multi-Object Tracker

The recent trend in vision-based multi-object tracking (MOT) is heading towards leveraging the representational power of deep learning to jointly learn to detect and track objects. However, existing methods train only certain sub-modules using loss functions that often do not correlate with established tracking evaluation measures such as Multi-Object Tracking Accuracy (MOTA) and Precision (MOTP). As these measures are not differentiable, the choice of appropriate loss functions for end-to-end training of multi-object tracking methods is still an open research problem. In this paper, we bridge this gap by proposing a differentiable proxy of MOTA and MOTP, which we combine in a loss function suitable for end-to-end training of deep multi-object trackers. As a key ingredient, we propose a Deep Hungarian Net (DHN) module that approximates the Hungarian matching algorithm. DHN allows estimating the correspondence between object tracks and ground truth objects to compute differentiable proxies of MOTA and MOTP, which are in turn used to optimize deep trackers directly. We experimentally demonstrate that the proposed differentiable framework improves the performance of existing multi-object trackers, and we establish a new state of the art on the MOTChallenge benchmark. Our code is publicly available from https://github.com/yihongXU/deepMOT.

==> How To Train Your Deep Multi-Object Tracker-camera_ready/tab/DHN_supp_testset.tex <==
\begin{table}
\tabcolsep=0.11cm
\centering
    \begin{center}
     \resizebox{\columnwidth}{!}{
        \begin{tabular}{c|c|ccc}
        \toprule
        Discretization & Network & WA \% ($\uparrow$) & MA\% ($\downarrow$)& SA\% ($\downarrow$) \\
        \midrule
        \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Row-wise \\ maximum\end{tabular}}}
        &\textbf{seq\_gru (proposed)}& \textbf{92.88}  & \textbf{4.79} & 3.39 \\
        &\textbf{seq\_lstm} & 83.66 & 13.79 &5.98  \\
        &\textbf{paral\_gru}& 89.56  & 8.21 & 4.99 \\
        &\textbf{paral\_lstm}& 88.93 & 8.67& 5.38\\
        &\textbf{1d\_conv}& 56.43 & 35.06& \textbf{2.78}\\ \midrule
        \midrule
        \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Column-wise \\ maximum\end{tabular}}}
        &\textbf{seq\_gru (proposed)}& \textbf{93.49} & \textbf{6.41} & 26.57 \\
        &\textbf{seq\_lstm} & 87.07 & 13.54 & 47.04\\
        &\textbf{paral\_gru}& 91.01& 7.98& 46.25\\
        &\textbf{paral\_lstm}& 90.50 & 8.60& 47.43 \\
        &\textbf{1d\_conv}& 56.18 & 79.54& \textbf{7.73} \\
        \bottomrule
        \end{tabular}
        }
    \end{center}
\caption{Evaluation results: comparison of different network structures and settings in terms of WA, MA and SA on the DHN test set.}\label{table:results-DHN-testset}
\end{table}

==> How To Train Your Deep Multi-Object Tracker-camera_ready/tab/DHN_supp_trainMat.tex <==
\begin{table}
\centering
\tabcolsep=0.11cm
    \begin{center}
     \resizebox{\columnwidth}{!}{
        \begin{tabular}{c|c|ccc}
        \toprule
        Discretization & Network & WA \% ($\uparrow$) & MA\% ($\downarrow$)& SA\% ($\downarrow$) \\
        \midrule
        \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Row-wise \\ maximum\end{tabular}}}
        &\textbf{seq\_gru (proposed)}& \textbf{92.71}  & \textbf{13.17} & 9.70 \\
        &\textbf{seq\_lstm} & 91.64 & 14.55 & 10.37  \\
        &\textbf{paral\_gru}& 86.84  & 23.50 & 17.15 \\
        &\textbf{paral\_lstm}& 71.58 & 42.48& 22.62\\
        &\textbf{1d\_conv}& 83.12 & 32.73 & \textbf{5.73} \\ \midrule
        \midrule
        \multicolumn{1}{c|}{\multirow{5}{*}{\begin{tabular}[c]{@{}c@{}}Column-wise \\ maximum\end{tabular}}}
        &\textbf{seq\_gru (proposed)}& \textbf{92.36} & \textbf{12.21} & 3.69 \\
        &\textbf{seq\_lstm} & 91.93 & 13.15 & 4.71\\
        &\textbf{paral\_gru}&87.24 & 20.56 & 16.67\\
        &\textbf{paral\_lstm}& 72.58 & 39.55& 23.16 \\
        &\textbf{1d\_conv}& 82.74 & 32.94 & \textbf{1.11} \\
        \bottomrule
        \end{tabular}
        }
    \end{center}
\caption{Evaluation results. Comparison of different network structures and settings in terms of WA, MA and SA on distance matrices during training.}\label{table:results-DHN-train-matrices}
\end{table}


==> How To Train Your Deep Multi-Object Tracker-camera_ready/tab/mot.tex <==

\begin{table}
\center
\tabcolsep=0.11cm

    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c l c c c c c c c c c}
    \toprule
     & Method & MOTA $\uparrow$ & MOTP $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$ \\ [0.5ex] 
     \midrule
     
     \parbox[t]{3mm}{\multirow{10}{*}{\rotatebox[origin=c]{90}{MOT17}}}
        & \method-Tracktor & \textbf{53.7} & 77.2 & 53.8  & 19.4  & 36.6  & \textbf{11731}  & 247447 & 1947  \\
        & Tracktor~\cite{Bergmann19ICCV} & 53.5  & 78.0 & 52.3 & 19.5 & 36.6 & 12201 & 248047 & 2072\\\cmidrule{2-10}
        & \method-SiamRPN & 52.1 & \textbf{78.1} & 47.7 & 16.7 & 41.7 & 12132 & 255743 & 2271 \\
        & SiamRPN~\cite{Li18CVPRb} & 47.8 & 76.4 & 41.4 & 17.0 & 41.7 & 38279 & 251989 & 4325 \\\cmidrule{2-10}
        & \method-GOTURN & 48.1 & 77.9 & 40.0 & 13.6 & 43.5 & 22497 & 266515 & 3792 \\
        & GOTURN~\cite{Held16ECCV}  & 38.3 & 75.1 & 25.7 & 9.4 & 47.1 & 55381 & 282670 & 10328 \\\cmidrule{2-10}
        & eHAF~\cite{Sheng18TCVSb} & 51.8 & 77.0 & \textbf{54.7} & \textbf{23.4} & 37.9 & 33212 & \textbf{236772} & 1834 \\
        & FWT~\cite{Henschel17arXiv} & 51.3 & 77.0 & 47.6 & 21.4 & \textbf{35.2} & 24101 & 247921 & 2648 \\
        & jCC~\cite{Keuper18TPAMI} & 51.2 & 75.9 & 54.5   & 20.9 & 37.0 & 25937 & 247822 & \textbf{1802} \\
        & MOTDT17~\cite{Long18ICME} & 50.9 & 76.6 & 52.7 & 17.5 & 35.7 & 24069 & 250768 & 2474 \\
        & MHT\_DAM~\cite{Kim15ICCV} & 50.7 & 77.5 & 47.2 & 20.8 & 36.9 & 22875 & 252889 & 2314 \\
     \midrule
     \midrule
     \parbox[t]{3mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{MOT16}}}
        & \method-Tracktor & \textbf{54.8} & 77.5 & \textbf{53.4} & \textbf{19.1} & \textbf{37.0} & \textbf{2955} & \textbf{78765} & 645  \\
        & Tracktor~\cite{Bergmann19ICCV} & 54.4 & 78.2 & 52.5 & 19.0 & 36.9 & 3280 & 79149 & 682 \\\cmidrule{2-10} 
        & \method-SiamRPN & 51.8 & 78.1 & 45.5 & 16.1 & 45.1 & 3576 & 83699 & 641 \\
        & SiamRPN~\cite{Li18CVPRb} & 44.0 & 76.6 & 36.6 & 15.5 & 45.7 & 18784 & 82318 & 1047 \\\cmidrule{2-10}
        & \method-GOTURN & 47.2 & 78.0 & 37.2 &13.7 & 46.1 & 7230 & 87781 & 1206 \\
        & GOTURN~\cite{Held16ECCV}  & 37.5 & 75.4 & 25.1 & 8.4 & 46.5 & 17746 & 92867 & 3277 \\\cmidrule{2-10}
        & HCC~\cite{Ma18ACCV} & 49.3 & \textbf{79.0} & 50.7 & 17.8 & 39.9 & 5333 & 86795 & \textbf{391} \\
        & LMP~\cite{Tang17CVPR} & 48.8 &\textbf{79.0} & 51.3 & 18.2 & 40.1 & 6654 & 86245 & 481 \\
        & GCRA~\cite{Ma18ICME} & 48.2 & 77.5 & 48.6 & 12.9 & 41.1 & 5104 & 88586 & 821 \\
        & FWT~\cite{Henschel17arXiv} & 47.8 & 75.5 & 44.3 & \textbf{19.1} & 38.2 & 8886 & 85487 & 852 \\
        & MOTDT~\cite{Long18ICME} & 47.6 &74.8 & 50.9 & 15.2 & 38.3 & 9253 & 85431 & 792 \\
    \bottomrule
    \end{tabular}
    }

\caption{We establish a new state-of-the-art on MOT16 and MOT17 public benchmarks by using the proposed DeepMOT.}
\label{tab:mot}
\end{table}

==> How To Train Your Deep Multi-Object Tracker-camera_ready/tab/mot15.tex <==

\begin{table}
\center
\tabcolsep=0.11cm

    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c l c c c c c c c c c}
    \toprule
     & Method & MOTA $\uparrow$ & MOTP $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$ \\ [0.5ex] 
     \midrule
     \parbox[t]{3mm}{\multirow{11}{*}{\rotatebox[origin=c]{90}{2D MOT 2015}}}
        & \method-Tracktor & \textbf{44.1}& \textbf{75.3} & 46.0 & 17.2 & 26.6 & 6085 & 26917 & 1347 \\
        & Tracktor~\cite{Bergmann19ICCV} & \textbf{44.1} & 75.0  & 46.7 & 18.0 & \textbf{26.2} & 6477 & \textbf{26577} & 1318 \\\cmidrule{2-10}
        & \method-SiamRPN & 33.3  & 74.6 & 32.7 & 9.3 & 43.7 & 7825 & 32211 & 919 \\
        & SiamRPN~\cite{Li18CVPRb} & 31.0 & 73.9& 30.7 & 12.6 & 41.7 & 10241 & 31099 & 1062 \\\cmidrule{2-10}
        & \method-GOTURN  & 29.8  & \textbf{75.3} & 27.7 & 4.0 & 66.6 & 3630 & 38964 & 524 \\
        & GOTURN~\cite{Held16ECCV}  & 23.9 & 72.8 & 22.3 & 3.6 & 66.4 & 7021 & 38750 & 965 \\\cmidrule{2-10}
        & AP\_HWDPL\_p~\cite{Chen17ICIP} & 38.5  & 72.6 & \textbf{47.1} & 8.7 & 37.4 & \textbf{4005} & 33203 & 586 \\
        & AMIR15~\cite{Sadeghian17ICCV} & 37.6  & 71.7 & 46.0 & 15.8 & 26.8 & 7933 & 29397 & 1026 \\
        & JointMC~\cite{Keuper18TPAMI} & 35.6  & 71.9& 45.1 & \textbf{23.2} & 39.3 & 10580 & 28508 & 457 \\
        & RAR15pub~\cite{Fang18WACV} & 35.1  & 70.9& 45.4 & 13.0 & 42.3 & 6771 & 32717 & \textbf{381} \\
    \bottomrule
    \end{tabular}
    }

\caption{Results on MOTChallenge MOT15 benchmark.}
\label{tab:mot15}
\end{table}

==> How To Train Your Deep Multi-Object Tracker-camera_ready/tab/mot_ablation.tex <==

\begin{table}
\center
\tabcolsep=0.11cm
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c l c c c c c c c c c}
    \toprule
     & Method & MOTA $\uparrow$ & MOTP $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$ \\ [0.5ex] 
     \midrule
     \parbox[t]{3mm}{\multirow{2}{*}{\rotatebox[origin=c]{90}{\footnotesize{Van.}}}} 
        & Base & 59.97 & 89.50 & 70.84 & 35.13 & 27.66 & 276 & 31827 & 326 \\
        & +ReIDext & \textbf{60.20} & \textbf{89.50} &  \textbf{71.15} & \textbf{35.13} & \textbf{27.80}  & \textbf{276}  & \textbf{31827}  & \textbf{152}  \\
        \midrule
        \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize{\method}}}} 
        & Base & 60.43 & 91.82 & 71.44 & 35.41 & 27.25 & 218 & 31545 & 309 \\
        & +ReIDext & 60.62 & 91.82 & 71.66 & 35.41 & 27.39 & 218 & 31545 & 149 \\ 
        & +ReIDhead & \textbf{60.66} & \textbf{91.82} & \textbf{72.32} & \textbf{35.41} & \textbf{27.25} & \textbf{218} & \textbf{31545} &\textbf{118} \\ 
    \bottomrule
    \end{tabular}
    }

\caption{Impact of the different ReID strategies for the two training strategies on Tracktor's performance.}
\label{tab:mot_ablation_modules}

\end{table}

==> How To Train Your Deep Multi-Object Tracker-camera_ready/tab/mot_sot_ablation.tex <==

\begin{table}
\center
\tabcolsep=0.11cm
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{c l c c c c c c c c c}
    \toprule
     & Training & MOTA $\uparrow$ & MOTP $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$ \\ [0.5ex] 
     \midrule
        \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize{GOTURN}}} }

        & Pre-trained & 45.99 & 85.87 & 49.83  & 22.27 & 36.51 & 2927 & 39271 & 1577 \\        
        & Smooth $L_1$ & 52.28 & 90.56 & 63.53 & \textbf{29.46} & \textbf{34.58} & 2026 & 36180 & 472  \\        
        & \method & \textbf{54.09} & \textbf{90.95} & \textbf{66.09} & 28.63 & 35.13 & \textbf{927} & \textbf{36019} & \textbf{261} \\        
        \midrule
        \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize{SiamRPN}}}}         
        & Pre-trained & 55.35 & 87.15 &66.95 & 33.61 & \textbf{31.81} & 1907 & 33925 & 356 \\   
        & Smooth $L_1$ & 56.51 & \textbf{90.88} & 68.38 & \textbf{33.75} &32.64 & 925 &  34151 & 167 \\  
        & \method & \textbf{57.16} & 89.32 & \textbf{69.49} & 33.47 & 32.78 & \textbf{889} &\textbf{33667} & \textbf{161} \\ 
        
        \midrule
        \parbox[t]{3mm}{\multirow{3}{*}{\rotatebox[origin=c]{90}{\footnotesize{Tracktor}}}}         
        & Vanilla  & 60.20 & 89.50 &  71.15 & 35.13 & 27.80  & 276  & 31827  & 152  \\
        & Smooth $L_1$ & 60.38 & 91.81 & 71.27 & 34.99 & 27.25 & 294 & 31649 & 164 \\ 
        & \method  & \textbf{60.66} & \textbf{91.82} & \textbf{72.32} & \textbf{35.41} & \textbf{27.25} & \textbf{218} & \textbf{31545} &\textbf{118} \\
    \bottomrule
    \end{tabular}
    }

\caption{DeepMOT vs.~Smooth $L_1$ using MOT-by-SOT baselines and Tracktor.}
\label{tab:mot_sot_ablation}
\end{table}

==> How To Train Your Deep Multi-Object Tracker-camera_ready/tab/mot_tracktor_ablation_loss.tex <==

\begin{table}
\center
\tabcolsep=0.11cm
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l c c c c c c c c c}
    \toprule
     Training loss & MOTA $\uparrow$ &  MOTP $\uparrow$ & IDF1 $\uparrow$ & MT $\uparrow$ & ML $\downarrow$ & FP $\downarrow$ & FN $\downarrow$ & IDS $\downarrow$ \\ [0.5ex] 
     \midrule
        Vanilla  & 60.20 & 89.50 &  71.15 & 35.13 & 27.80  & 276  & 31827  & 152  \\
        Smooth $L_1$ & 60.38 & 91.81 & 71.27 & 34.99 & 27.25 & 294 & 31649 & 164 \\ 
        \midrule
        $\diffmotp$ & 60.51 & 91.74 & 71.75 & 35.41 & \textbf{26.83} & 291 & 31574 & 142\\
        $\diffmota$ &  60.52 &  88.31 &  71.92 &  35.41 &  27.39 &  254 &  31597 &  142 \\   
        $\diffmota$+$\diffmotp$-$\diffids$ & 60.61  & \textbf{92.03} & 72.10  & 35.41  & 27.25  & 222  & 31579  & 124 \\
        
        $\diffmota$+$\diffmotp$ & \textbf{60.66} & 91.82 & \textbf{72.32} & \textbf{35.41} & 27.25 & \textbf{218} & \textbf{31545} &\textbf{118}  \\
        
        
    \bottomrule
    \end{tabular}
    }

\caption{Ablation study on the effect the training loss on Tracktor.}
\label{tab:mot_tracktor_ablation_loss}

\end{table}
